CamoDiffusion: Camouflaged Object Detection via Conditional Diffusion Models

Camouflaged Object Detection (COD) is a challenging task in computer vision due to the high similarity between camouflaged objects and their surroundings. Existing COD methods primarily employ semantic segmentation, which suffers from overconfident incorrect predictions. In this paper, we propose a new paradigm that treats COD as a conditional mask-generation task leveraging diffusion models. Our method, dubbed CamoDiffusion, employs the denoising process of diffusion models to iteratively reduce the noise of the mask. Due to the stochastic sampling process of diffusion, our model is capable of sampling multiple possible predictions from the mask distribution, avoiding the problem of overconfident point estimation. Moreover, we develop specialized learning strategies that include an innovative ensemble approach for generating robust predictions and tailored forward diffusion methods for efficient training, specifically for the COD task. Extensive experiments on three COD datasets attest the superior performance of our model compared to existing state-of-the-art methods, particularly on the most challenging COD10K dataset, where our approach achieves 0.019 in terms of MAE.

==> table_or_algo/Tab-Hyper-Parameter-Setting.tex <==
\begin{table}[t!]
  % \vspace{-10pt}
  \footnotesize
  \centering
  \small{
    \caption{Quantitative results of our proposed \ourmodel\ with different hyperparameters, including the number of sampling time steps and SNR shift.The best result is marked in bold.}\label{tab:hyper-parameterSetting}
  }
  % \vspace{-10pt}
  \renewcommand{\arraystretch}{0.4}
  \setlength\tabcolsep{11.0pt}
% \begin{tabular}{ll|cccc}
  \begin{tabular}{lrcccc}
  %\hline
  \toprule&
  &\multicolumn{4}{c}{\tabincell{c}{COD10K~\cite{fan2020camouflaged}}}  \\
   \cmidrule(lr){3-6}
   Sample Time Steps ~~~ &SNR Shift  &$S_\alpha\uparrow$      &$E_\phi\uparrow$     &$F_\beta^w\uparrow$      &$M\downarrow$\\ \hline
   1 & $-2\log(5.5)$ & 0.873 & 0.940 &0.806 &0.021 \\
   2 & $-2\log(5.5)$ & 0.875 & 0.943 &0.812 &0.020 \\
   3 & $-2\log(5.5)$ & 0.878 & 0.942 &0.812 &0.020 \\
   5 & $-2\log(5.5)$ & 0.880 & 0.942 &0.813 &0.020 \\
   10 & $-2\log(5.5)$& 0.880 & \textbf{0.943} &0.815 &\textbf{0.020} \\
   20 & $-2\log(5.5)$& \textbf{0.881} & \textbf{0.943} &\textbf{0.816} &\textbf{0.020} \\
   \hline
   10 & $-2\log(1)$ &0.855 &0.922 &0.767 &0.024 \\
   10 & $-2\log(3)$ &0.872 &0.938 &0.798 &0.022\\
   10 & $-2\log(5.5)$& \textbf{0.880} & \textbf{0.943} &\textbf{0.815} &\textbf{0.020} \\
   10 & $-2\log(12)$ &0.874 &0.937 &0.803 &0.021 \\
   
  %\hline
\bottomrule
  \end{tabular}
  \vspace{-3mm}
\end{table}  
